On Feller Continuity and Full Abstraction (Long Version)

We study the nature of applicative bisimilarity in $\lambda$-calculi endowed with operators for sampling from continuous distributions. On the one hand, we show that bisimilarity, logical equivalence, and testing equivalence all coincide with contextual equivalence when real numbers can be manipulated only through continuous functions. The key ingredient towards this result is a novel notion of Feller-continuity for labelled Markov processes, which we believe of independent interest, being a broad class of LMPs for which coinductive and logically inspired equivalences coincide. On the other hand, we show that if no constraint is put on the way real numbers are manipulated, characterizing contextual equivalence turns out to be hard, and most of the aforementioned notions of equivalence are even unsound.

==> macros.tex <==

%\newtheorem{notation}{Notation}
%\newtheorem{remark}{Remark}

\newcommand{\hide}[1]{}
\newcommand{\remarque}[1]{\textcolor{blue}{\ifthenelse{\equal{\withcomments}{1}}{#1}{}}}
\newcommand{\ugo}[1]{\textcolor{green}{\ifthenelse{\equal{\withcomments}{1}}{#1}{}}}
\newcommand{\francesco}[1]{\textcolor{red}{\ifthenelse{\equal{\withcomments}{1}}{#1}{}}}
\newcommand{\gb}[1]{\textcolor{green}{\ifthenelse{\equal{\withcomments}{1}}{#1}{}}}
\newcommand{\TODO}[1]{\textcolor{red}{\ifthenelse{\equal{\withcomments}{1}}{#1}{}}}
\RequirePackage{ifthen}
\newcommand{\typeof}{1} % 0 is for short verion, 1 is for long version
\newcommand{\longv}[1]{\ifthenelse{\equal{\typeof}{0}}{}{#1}}
\newcommand{\shortv}[1]{\ifthenelse{\equal{\typeof}{0}}{#1}{}}
\newcommand{\withcomments}{0} % 1 is to get comments, 0 is not to have them.


\newcommand{\norm}[1]{\lVert #1 \rVert}

\newcommand{\tor}[1]{ \stackrel{#1}{\to}}
\newcommand{\torr}[2]{{ \stackrel{#1 \leadsto #2}{\to}}}
\newcommand{\variables}{\mathbf{V}}

\newcommand{\forget}[1]{\overline{#1}}
\newcommand{\domain}[1]{\text{Dom}(#1)}
\newcommand{\cdomain}[1]{\text{CDom}(#1)}

\newcommand{\interior}[1]{\mathring{#1}}
\newcommand{\interiorr}[2]{\mathring{#2}^{#1}}
\newcommand{\safep}[1]{\mathcal{SP}(#1)}
\newcommand{\criticalp}[1]{\mathcal{CP}(#1)}

\newcommand{\neighbor}[3]{\mathcal V^{#1}(#2,#3)}

\newcommand{\voidtype}{\mathbf{void}}
\newcommand{\unittype}{\mathbf{unit}}
\newcommand{\booltype}{\mathbf{bool}}
\newcommand{\trueval}{\mathbf{true}}
\newcommand{\falseval}{\mathbf{false}}
\newcommand{\ite}[3]{\textbf{if}\ #1\ \textbf{then}\ #2\ \textbf{else}\ #3}

\newcommand{\nattype}{\mathbf{nat}}
\newcommand{\lebesgue}{\lambda}
\newcommand{\subst}[3]{#1[#3/#2]}
\newcommand{\reals}{\mathbf{R}}
\newcommand{\probb}{\mathbf{P}}

%% TERMS, EVALUATION %%% -> TO BE ORDERED AND COMPLETED
%\newcommand{\closedTerms}{\terms_0}
%\newcommand{\closedValues}{\values_0}
%\newcommand{\reloneTerms}{\relone^{\terms}}
\newcommand{\reloneValues}{\relone^{\values}}
%\newcommand{\relthreeTerms}{\relthree_{\terms}}
\newcommand{\relthreeValues}{\relthree_{\values}}
%\newcommand{\terms}{\Lambda}
\newcommand{\values}{\mathscr{V}}
%\newcommand{\terms}{\Lambda}
\newcommand{\hnf}{\mathsf{H}}
\newcommand{\scr}[1]{\,{#1}^{SC}\,}
\newcommand{\dom}[1]{\,\mathit{dom}(#1)\,}
\newcommand{\ttrue}{\,\mathsf{true}\,}
\newcommand{\ffalse}{\,\mathsf{false}\,}
\newcommand{\bbool}{\,\mathsf{bool}\,}
\newcommand{\nil}{\,\mathsf{nil}\,}
\newcommand{\evav}[1]{#1 \Downarrow}
%\newcommand{\eval}[2]{#1 \Downarrow_n #2}
\newcommand{\evalv}[2]{#1 \Downarrow \distr{#2}}
\newcommand{\evalvp}[2]{#1 \Downarrow^{#2}}
\newcommand{\evalvs}[2]{#1 \Rightarrow {\distr{#2}}}
\newcommand{\evalvsD}[2]{#1 \Rightarrow {{#2}}}
\newcommand{\evalvsp}[2]{#1 \Rightarrow^{#2}}
\newcommand{\distrv}[1]{{\{{#1}^1\}}}
\newcommand{\distrav}[1]{\{ {{#1}^{1}} \}}
\newcommand{\distr}[1]{\mathscr #1}
\newcommand{\diS}[1]{\llbracket #1\rrbracket}
\newcommand{\fixe}[1]{\widetilde{\mathsf{fix}}[#1]}
\newcommand{\fixi}[2]{\widetilde{\mathsf{fix}^{#1}}[#2]}
%\newcommand{\op}[2]{#1 \, \mathsf{op}\, #2}
\newcommand{\opn}[2]{#1 \, \tilde {\mathsf{op}}\, #2}
%\newcommand{\fst}[1]{\mathsf{fst}\, (#1)}
%\newcommand{\snd}[1]{\mathsf{snd}\, (#1)}
\newcommand{\abstrac}{\lambda x.}
\newcommand{\abstr}[2]{\lambda #1.#2}
\newcommand{\ifth}[3]{\mathbf{if}\, #1\,  \mathbf{then} \,#2 \,\mathbf{else}\, 
#3}
\newcommand{\fix}[2]{\mathbf{fix}\ #1.#2}
\newcommand{\pair}[2]{\langle #1,#2 \rangle}
\newcommand{\caset}[3]{\mathsf{case}\, #1\, \mathsf{of}\, \{ 
\mathsf{nil}\rightarrow #2\;|\;h::t \rightarrow #3\}}
\newcommand{\lst}[2]{#1 :: #2}
\newcommand{\id}{1}
\newcommand{\termty}[1]{\mathcal{T}^{#1}}
%\newcommand{\val}[1]{\mathcal{V}^{#1}}
\newcommand{\termtyg}[2]{\mathcal{T}_{#1}^{#2}}
\newcommand{\R}{{\precsim^n_\circ}}
\newcommand{\E}{{\backsim^n_\circ}}
\newcommand{\Rh}{{{\precsim^n_\circ}^H}}
\newcommand{\Inf}[3]{#1\,{{\precsim^n_\circ}^H}_{#1}\,#3}
\newcommand{\Rv}{{\precsim_\circ}}
\newcommand{\Ev}{{\backsim_\circ}}
\newcommand{\Rvh}{\precsim_\circ^H}
\newcommand{\LOP}{\ensuremath{\Lambda_\oplus}}
\newcommand{\PCF}{\ensuremath{\mathsf{PCF}}}
\newcommand{\PCFL}{\ensuremath{\mathsf{PCFL}}}
\newcommand{\PCFLP}{\ensuremath{\mathsf{PCFL}_\oplus}}
\newcommand{\varone} {x}
\newcommand{\vartwo} {y}
\newcommand{\varthree} {z}
\newcommand{\termone}{M}
\newcommand{\termtwo}{N}
\newcommand{\termthree}{L}
\newcommand{\expr}{e}
\newcommand{\termoneone}{\expr_{1}}
\newcommand{\termonetwo}{\expr_{2}}
\newcommand{\termonethree}{\expr_{3}}
\newcommand{\termonefour}{\expr_{4}}
\newcommand{\subterm}[2]{\mbox{\tt{#1_{#2}}}}
\newcommand{\ectctxone}{\varepsilon}
\newcommand{\app}[2]{#1 \mathbin{\ast} #2}
\newcommand{\termfour}{h}
\newcommand{\termfive}{g}
\newcommand{\termsix}{Z}
\newcommand{\termseven}{Y}
\newcommand{\termeight}{r}
\newcommand{\emb}[1]{\langle\!\langle #1\rangle\!\rangle}
\newcommand{\embsn}[1]{\lceil #1\rceil}
\newcommand{\abstrsv}[1]{\lambda.#1}
\newcommand{\dmyval}{\star}
\newcommand{\fixt}{\mathsf{fix}}
\newcommand{\fv}[1]{FV(#1)}
\newcommand{\env}{\Gamma}
\newcommand{\envone}{\env}
\newcommand{\envtwo}{\Delta}
\newcommand{\vars}{\vec{\varone}}
\newcommand{\imp}{\vdash}
\newcommand{\raiseExcep}[1]{\mathsf{raise}_{#1}}
%\newcommand{\complexitycomp}{c_\terms}
\newcommand{\complexityval}{c_\values}
\newcommand{\constructor}{\theta}
\newcommand{\constructortype}{\vartheta}


%%% LAMBDA CALCULUS %%%
\newcommand{\abs}[2]{\lambda #1.#2}
\newcommand{\letin}[3]{\texttt{let }#1=#2\texttt{ in }#3}
\newcommand{\valone}{V}
\newcommand{\valtwo}{W}
\newcommand{\valthree}{U}
\newcommand{\valfour}{Z}
\newcommand{\valset}{\mathscr{V}}
\newcommand{\valsettwo}{\mathscr{W}}
\renewcommand{\terms}{\mathscr{T}}
\newcommand{\programs}{\mathscr{P}}
\newcommand{\typeone}{\sigma}
\newcommand{\typetwo}{\tau}
\newcommand{\typethree}{\iota}
\newcommand{\types}{T}
\newcommand{\typetarget}{T^t}
\newcommand{\typesource}{T^s}
\newcommand{\typeonea}{A}
\newcommand{\typetwoa}{B}
\newcommand{\typethreea}{C}
\newcommand{\funsymbol}{f}
\newcommand{\funsymbols}{\mathfrak{F}}
\newcommand{\fsone}{f}	
\newcommand{\funpred}{\mathcal{F}}
\newcommand{\rnone}{r}

%%% NOTATION %%%
\newcommand{\midd}{\;\;\mbox{\Large{$\mid$}}\;\;}

\newcommand{\derivfun}{\mathfrak{D}}

\newcommand{\diffset}{\mathcal{D}}

\newcommand{\makereal}[1]{\bm{#1}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb N}
\newcommand{\typereal}{\mathbf{real}}
\newcommand{\dtypereal}{\texttt{R}^{d}}
\newcommand{\typenat}{N}
\newcommand{\judgone}{j}
\newcommand{\set}{\mathbf{Set}}
\newcommand{\comp}{\circ}
\newcommand{\lambdareal}{\Lambda^{\mathsf{Real}}}
\newcommand{\logpred}[1]{\llparenthesis #1 \rrparenthesis}
\newcommand{\impr}{\, \vdash_{r} \,}
\newcommand{\imprr}[2]{\, \stackrel{#1 \leadsto #2}{\vdash_{r}} \,}
\newcommand{\imprh}[1]{\, \stackrel{#1}{\vdash_{r}} \,}
\newcommand{\impdr}[2]{\, \stackrel{#1 \leadsto #2}{\vdash_{D}} \,}
\newcommand{\impdh}[1]{\, \stackrel{#1}{\vdash_{D}} \,}
\newcommand{\hh}{\hdots}
\newcommand{\cc}{\cdots}
\newcommand{\bnf}{\;::=\;}
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\defeq}{\triangleq}
\newcommand{\open}[1]{#1^{\mathsf{open}}}
\newcommand{\support}[1]{\mathsf{supp}(#1)}
\newcommand{\red}[2]{RED^{#1}_{#2}}

\newcommand{\tcone}{\mathcal C}

\newcommand{\gpart}[1]{\,G #1\,}
\newcommand{\hpart}[1]{\,H #1 \,}

%% Generalized Typing judgments
\newcommand{\gendone}{\mathbf{O}}
\newcommand{\gendtwo}{\mathbf{U}}

\newcommand{\contpred}{\mathcal{C}}
\newcommand{\redgr}[4]{\contpred (#1, {#2 \leadsto #3},#4)}
\newcommand{\redgh}[3]{\contpred(#1, #2,#3)}

\newcommand{\fst}[1]{#1.1} 
\newcommand{\snd}[1]{#1.2}
\newcommand{\ith}[1]{#1.i}
\newcommand{\envreal}{\Theta}
\newcommand{\substone}{\gamma}
\newcommand{\substtwo}{\delta}

\newcommand{\de}[1]{\mathit{d} #1}
\newcommand{\devar}[1]{\mathtt{d} #1}
\newcommand{\val}[1]{\mathcal{V}[#1]}
\newcommand{\tangent}[1]{\mathcal{T}[#1]}
\newcommand{\dual}[2]{\mathtt{dual}_{#1}(#2)}
\newcommand{\deriv}[2]{\mathtt{deriv}(#1,#2)}
\newcommand{\Lambdacont}{{\Lambda_{\probb}^c}}
\newcommand{\Lambdadiff}{\Lambda_{\textnormal{d}}}

\newcommand{\relone}{\mathcal{R}}
\newcommand{\reltwo}{\mathcal{S}}
\newcommand{\idrel}{\mathcal{I}}


\newcommand{\rels}{\mathscr R}
\newcommand{\vect}[1]{\vec{#1}}
\newcommand{\dfunbeta}{(\textsf{D-fun}_\beta)}
\newcommand{\dfun}{(\textsf{D-fun})}
\newcommand{\dappbeta}{(\textsf{D-app}_\beta)}
\newcommand{\dappleft}{(\textsf{D-app}_l)}
\newcommand{\dappright}{(\textsf{D-app}_r)}
\newcommand{\dpairbetaleft}{(\textsf{D-pair}_{\beta_{1}})}
\newcommand{\dpairbetaright}{(\textsf{D-pair}_{\beta_{2}})}
\newcommand{\dpairleft}{(\textsf{D-pair}_l)}
\newcommand{\dpairright}{(\textsf{D-pair}_r)}
\newcommand{\dprojleft}{(\textsf{D-1})}
\newcommand{\dprojright}{(\textsf{D-2})}
\newcommand{\dpairbetaith}{(\textsf{D-pair}_{\beta_{i}})}

\newcommand{\dopenfunbeta}{(\textsf{D$^o$-fun}_\beta)}
\newcommand{\dopenfun}{(\textsf{D$^o$-fun})}
\newcommand{\dopenappbeta}{(\textsf{D$^o$-app}_\beta)}
\newcommand{\dopenappleft}{(\textsf{D$^o$-app}_l)}
\newcommand{\dopenappright}{(\textsf{D$^o$-app}_r)}
\newcommand{\dopenpairbetaleft}{(\textsf{D$^o$-pair}_{\beta_{1}})}
\newcommand{\dopenpairbetaright}{(\textsf{D$^o$-pair}_{\beta_{2}})}
\newcommand{\dopenpairleft}{(\textsf{D$^o$-pair}_l)}
\newcommand{\dopenpairright}{(\textsf{D$^o$-pair}_r)}
\newcommand{\dopenprojleft}{(\textsf{D$^o$-1})}
\newcommand{\dopenprojright}{(\textsf{D$^o$-2})}
\newcommand{\dopenpairbetaith}{(\textsf{D$^o$-pair}_{\beta_{i}})}

\newcommand{\STLambda}{\Lambda^{\times, \to}}
\newcommand{\STLambdareal}{\Lambda^{\times, \to, \typereal}}
\newcommand{\STLambdarealfun}{\Lambda^{\times, \to, \typereal}_{\funsymbols}}
\newcommand{\STLambdarealcont}{\Lambda^{\times, \to, \typereal}_{\contfun}}
\newcommand{\STLambdarealderiv}{\Lambda^{\times, \to, \typereal}_{\derivfun}}


\newcommand{\ctheorem}{Containment Theorem}

%%% Probabilistic Constructs %%%%%%%%%%%%%
\newcommand{\sample}{\mathbf{sample}}
\newcommand{\ps}{\oplus}

%%% LMPs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\markovone}{\mathcal S}
\newcommand{\lmpone}{\mathcal M}
\newcommand{\lmponelambda}{\mathcal M_{\Lambda_{\probb}}}
\newcommand{\lmponelambdac}{\mathcal M_{\Lambda_{\probb}^c}}
\newcommand{\evalact}{\text{eval}}
\newcommand{\unboxact}{\text{unbox}}
\newcommand{\giry}{\mathcal G}
\newcommand{\actsone}{\mathcal A}
\newcommand{\actstwo}{\mathcal B}
\newcommand{\Logic}{\mathcal L}
\newcommand{\act}[3]{\langle#1\rangle_{#2}{#3}}
\newcommand{\relator}{\Gamma}

\newcommand{\tests}{\mathcal T}
\newcommand{\testone}{\alpha}
\newcommand{\testtwo}{\beta}
\newcommand{\probsucc}[2]{\text{Prob}(#1,#2)}
\newcommand{\rela}[1]{\relone_{#1}}
\newcommand{\relaop}[3]{#1 \, #2\,#3}
\newcommand{\relaasym}[1]{\mathscr R^{\rightarrow}({#1})}
\newcommand{\disting}[1]{\widehat{#1}}

\newcommand{\pLambda}{\Lambda_p}


\newcommand{\distrone}{\mu}
\newcommand{\distrtwo}{\nu}
\newcommand{\couplingone}{\pi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Categories
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Meas}{\textbf{Meas}}
\newcommand{\Pol}{\textbf{Pol}}
\newcommand{\Stbor}{\textbf{StBor}}
\newcommand{\Krn}{\textbf{Krn}}
\newcommand{\BLsigma}{\textbf{BL}_{\sigma}}
\newcommand{\tokrn}{\rightarrowtriangle}
\newcommand{\dirac}[1]{\{#1^{1}\}}
\newcommand{\Sp}{\mathcal S}
\newcommand{\lp}{L^1}
\newcommand{\normp}[2]{\norm{#1}^1_{#2}}
\newcommand{\distrs}[1]{\Delta{(#1)}}
\newcommand{\distrsp}[1]{\Delta^{=}{(#1)}}
\newcommand{\kernel}{\rightarrowtriangle}
\newcommand{\kernelp}{\rightarrowtriangle^{=}}

\newcommand{\lanone}{\Lambda}
\newcommand{\QQ}{\mathbb{Q}}

%Types and Terms
\newcommand{\typeOne}{\sigma}
\newcommand{\typeTwo}{\tau}
\newcommand{\typeThree}{\rho}
\newcommand{\atomicType}{a}
\newcommand{\typeVar}{t}
\newcommand{\typevar}{\alpha}
\newcommand{\zerotype}{\mathsf{void}}
\newcommand{\sumtype}[2]{\sum\nolimits_{#1}{#2}}
\newcommand{\typevarone}{t}
\newcommand{\recType}[2]{\mu #1.#2}
\newcommand{\rectype}[2]{\mu #1.#2}
\newcommand{\op}{\bm{f}}
\newcommand{\opone}{\bm{f}}
\newcommand{\optwo}{\bm{g}}
\newcommand{\boolfun}{b}
\newcommand{\Boolfun}{\mathcal{B}}



\newcommand{\functional}[1]{\lan #1 \ran}
%\newcommand{\seq}[2]{\mathbf{let}\ x = #1\ \mathbf{in}\ #2}
\newcommand{\seq}[2]{\mathbf{let}\ \varone = #1\ \mathbf{in}\ #2}
\newcommand{\seqlet}[2]{\mathbf{let}\ \varone = #1\ \mathbf{in}\ #2}
\newcommand{\seqlety}[2]{\mathbf{let}\ \vartwo = #1\ \mathbf{in}\ #2}

\newcommand{\seqto}[2]{#1\ \mathbf{to}\ \varone.#2}

\newcommand{\seqq}[2]{#1\ \mathbf{to}\ x.#2}
\newcommand{\seqy}[2]{\mathbf{let}\ \vartwo = #1\ \mathbf{in}\ #2}
\newcommand{\letpair}[2]{\mathsf{let}\ \lan x,y\ran\ = #1\ \mathsf{in}\ #2}
\renewcommand{\pair}[2]{\lan #1, #2 \ran}
\newcommand{\fold}[1]{\mathbf{fold}\ #1}
\newcommand{\letfold}[2]{\mathsf{let}\ \fold{x} = #1\ \mathsf{in}\ #2}
\newcommand{\tofold}[2]{#1\ \mathsf{to}\ \fold{x}.#2}
\newcommand{\topair}[2]{#1\ \mathsf{to}\ \lan x,y\ran.#2}
\newcommand{\pmpair}[2]{\mathsf{pm}\ #1\ \mathsf{as}\ 
	\pair{\varone}{\vartwo}.#2}
\newcommand{\casepair}[2]{\mathbf{case}\ #1\ \mathbf{of}\ 
	\{ \pair{\varone}{\vartwo} \to #2\}}
\newcommand{\inject}[2]{\langle #1, #2 \rangle}
\newcommand{\casesum}[2]{\mathbf{pm}\ #1\ \mathbf{as}\ 
	\inject{i}{\varone}. #2}
\newcommand{\casesumy}[2]{\mathbf{case}\ #1\ \mathbf{of}\ 
	\{\inject{i}{\vartwo} \to #2\}}
\newcommand{\unitval}{\lan \ran}
\newcommand{\caseunit}[2]{\mathbf{case}\ #1\ \mathbf{of}\ 
	\{ \unitval \to #2\}}
\newcommand{\unfoldin}[2]{\mathbf{case}\ #1\ \mathbf{of}\ 
	\{\fold{\varone} \to #2\}}
\newcommand{\unfold}[1]{\mathbf{unfold}\ #1}
\newcommand{\pmfold}[2]{\unfoldin{#1}{#2}}
\newcommand{\casefold}[2]{\unfoldin{#1}{#2}}
\newcommand{\casefoldy}[2]{\mathbf{case}\ #1\ \mathbf{of}\ \{\mathbf{fold}\ 
\vartwo \to #2\}}
\newcommand{\casefoldz}[2]{\mathbf{case}\ #1\ \mathbf{of}\ \{\mathbf{fold}\ 
\varthree \to #2\}}


\newcommand{\casefoldvar}[3]{\mathbf{case}\ #2\ \mathbf{of}\ \{ \mathbf{fold}\ 
#1 \to #3\}}

\newcommand{\unbang}[2]{\mathbf{case}\ #1\ \mathbf{of}\ 
	\{\bang \varone \to #2\}}
\newcommand{\casebang}[2]{\unbang{#1}{#2}}
\newcommand{\casebangy}[2]{\mathbf{case}\ #1\ \mathbf{of}\ \{ !\vartwo \to #2\}}
\newcommand{\casebangz}[2]{\mathbf{case}\ #1\ \mathbf{of}\ \{ !\varthree \to 
#2\}}

\newcommand{\pmbang}[2]{\unbang{#1}{#2}}
\newcommand{\pmbangy}[2]{\mathsf{pm}\ #1\ \mathsf{as}\ \bang{\vartwo}.#2}
\newcommand{\envOne}{\Gamma}
\newcommand{\envTwo}{\Delta}
\newcommand{\envThree}{\Theta}
\renewcommand{\envone}{\envOne}
\renewcommand{\envtwo}{\envTwo}
\newcommand{\envthree}{\envThree}
\newcommand{\emptyenv}{\emptyset}
\newcommand{\substType}[3]{#1[#3/#2]}
\newcommand{\substtype}[3]{#1[#2 := #3]}
%\renewcommand{\eval}[2]{\llbracket #2 \rrbracket_{#1}}
%\newcommand{\termdist}[1]{#1^{\terms}}
\newcommand{\valdist}[1]{#1^{\values}}
\newcommand{\numvalone}{v}
\newcommand{\numvaltwo}{w}
\newcommand{\numvalthree}{u}
\newcommand{\laxext}[1]{\hat{#1}}
\newcommand{\bisimdist}{\mathcal{B}}
\newcommand{\bdist}{\delta}
\newcommand{\qtensor}{\otimes}


\newcommand{\valseq}[2]{#1 \vdash^{\mathsf{v}} #2}
\newcommand{\compseq}[2]{#1 \compimp #2}
\newcommand{\howevalseq}[2]{#1 \Vdash^{\mathsf{v}} #2}
\newcommand{\howecompseq}[2]{#1 \Vdash^{\mathsf{c}} #2}
\newcommand{\howe}[1]{\mathbin{#1^{\scriptscriptstyle{H}}}}

\newcommand{\dd}{d}
\newcommand{\Graph}[1]{#1_{\circ}}
\newcommand{\strongkleisli}[1]{#1^{*}}
\newcommand{\catunit}{I}
\newcommand{\unitor}{\lambda}
\newcommand{\curry}{\mathsf{curry}}
\newcommand{\uncurry}{\mathsf{uncurry}}
\newcommand{\associator}{\alpha}
\newcommand{\leftunitor}{\lambda}
\newcommand{\rightunitor}{\rho}
\newcommand{\commutator}{\gamma}
\newcommand{\laxcommutegeq}{\ar @{} [dr] |\geq}
\newcommand{\laxcommute}{\ar @{} [dr] |\leq}
\newcommand{\laxcommuterel}{\ar @{} [dr] |\subseteq}
\newcommand{\commute}{\ar @{} [dr] |{=}}
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\divergence}{\Uparrow}
\newcommand{\partiality}[1]{#1_{\divergence}}
\newcommand{\effvalone}{e}
\newcommand{\substeff}[3]{#1\{#2 := #3\}}
\newcommand{\weight}{\omega}
\newcommand{\monadvalone}{t}
\newcommand{\monadvaltwo}{u}
\newcommand{\nf}{\mathsf{nf}}
%\newcommand{\constructor}[2]{\theta\{#1\}_{#2}}
\newcommand{\constructoR}{\theta}
\newcommand{\trivialrel}{\mathcal{U}}

\newcommand{\baseone}{s}
\newcommand{\basetwo}{r}
\newcommand{\basethree}{p}
\newcommand{\baseid}{1}
\newcommand{\bang}{{!}}
\newcommand{\quantalethree}{\mathcal{U}}

\newcommand{\toval}[1]{\mathbin{#1_{\scriptscriptstyle \values}}}
\newcommand{\toterm}[1]{\mathbin{#1_{\scriptscriptstyle \Lambda}}}
\newcommand{\towhnf}[1]{\mathbin{#1_{\scriptscriptstyle \Whnf}}}
\newcommand{\toenf}[1]{\mathbin{#1_{\scriptscriptstyle \Enf}}}
\newcommand{\howeval}[1]{\mathbin{#1^{\scriptscriptstyle{H}}_{\scriptscriptstyle
 \values}}}
\newcommand{\howeterm}[1]{\mathbin{#1^{\scriptscriptstyle{H}}_{\scriptscriptstyle
 \Lambda}}}

\newcommand{\ruleVar}{(\mathsf{var})}
\newcommand{\ruleReturn}{(\mathsf{val})}
\newcommand{\ruleSeq}{(\mathsf{let})}
\newcommand{\ruleApp}{(\mathsf{app})}
\newcommand{\ruleAbs}{(\mathsf{abs})}
\newcommand{\ruleInject}{(\mathsf{inj})}
\newcommand{\ruleCaseInject}{(\mathsf{inj}\text{-}\mathsf{cases})}
\newcommand{\rulePair}{(\tensor I)}
\newcommand{\ruleCasePair}{(\tensor E)}
\newcommand{\ruleFold}{(\mathsf{fold})}
\newcommand{\ruleCaseFold}{(\mathsf{fold}\text{-}\mathsf{cases})}
\newcommand{\ruleBang}{(\mathsf{bang})}
\newcommand{\ruleCaseBang}{(\mathsf{bang}\text{-}\mathsf{cases})}
\newcommand{\ruleUnbang}{(\mathsf{unbang})}
\newcommand{\ruleOp}{(\mathsf{op})}
%%%%%%%%%%%
\newcommand{\ruleEvalReturn}{(\mathsf{val}_\evalto)}
\newcommand{\ruleEvalSeq}{(\mathsf{let}_\evalto)}
\newcommand{\ruleEvalApp}{(\mathsf{app}_\evalto)}
\newcommand{\ruleEvalCaseInject}{(\mathsf{case}\text{-}\mathsf{inj}_\evalto)}
\newcommand{\ruleEvalCaseFold}{(\mathsf{case}\text{-}\mathsf{fold}_\evalto)}
\newcommand{\ruleEvalCaseBang}{(\mathsf{case}\text{-}\mathsf{bang}_\evalto)}
\newcommand{\ruleEvalOp}{(\mathsf{op}_\evalto)}
\newcommand{\ruleEvalBot}{(\bot_\evalto)}

%%%%%%%%%%%
\newcommand{\carrier}[1]{#1_0}
\newcommand{\sub}[2]{#1[#2]}
\newcommand{\howeimp}{\toterm{\models}}
\newcommand{\ruleHVar}{(\mathsf{H\text{-}var})}
\newcommand{\ruleHReturn}{(\mathsf{H\text{-}val})}
\newcommand{\ruleHSeq}{(\mathsf{H\text{-}let})}
\newcommand{\ruleHApp}{(\mathsf{H\text{-}app})}
\newcommand{\ruleHAbs}{(\mathsf{H\text{-}abs})}
\newcommand{\ruleHPair}{\mathsf{Howe\text{-}}(\tensor I)}
\newcommand{\ruleHPmPair}{\mathsf{Howe\text{-}}(\tensor E)}
\newcommand{\ruleHInject}{(\mathsf{H\text{-}inj})}
\newcommand{\ruleHCaseSum}{(\mathsf{H\text{-}sum\text{-}cases})}
\newcommand{\ruleHFold}{(\mathsf{H\text{-}fold})}
\newcommand{\ruleHPmFold}{(\mathsf{H\text{-}fold\text{-}cases})}
\newcommand{\ruleHBang}{(\mathsf{H\text{-}bang})}
\newcommand{\ruleHPmBang}{(\mathsf{H\text{-}bang\text{-}cases})}
\newcommand{\ruleHOp}{(\mathsf{H\text{-}op})}
\newcommand{\ruleHEctxNil}{(\mathsf{E\text{-}nil})}
\newcommand{\ruleHEctxApp}{(\mathsf{E\text{-}app})}
\newcommand{\ruleHEctxSeq}{(\mathsf{E\text{-}let})}

\newcommand{\ruleCompVar}{(\mathsf{comp\text{-}var})}
\newcommand{\ruleCompAbs}{(\mathsf{comp\text{-}abs})}
\newcommand{\ruleCompApp}{(\mathsf{comp\text{-}app})}
\newcommand{\ruleCompRet}{(\mathsf{comp\text{-}ret})}
\newcommand{\ruleCompSeq}{(\mathsf{comp\text{-}let})}
\newcommand{\ruleCompOp}{(\mathsf{comp\text{-}op})}


\newcommand{\kantorovich}{K}
\newcommand{\zero}{\ket{0}}

\newcommand{\valimp}{\imp^{\scriptscriptstyle{\values}}}
\newcommand{\compimp}{\imp^{\scriptscriptstyle{\terms}}}
\newcommand{\enfimp}{\imp^{\scriptscriptstyle{\Enf}}}
\newcommand{\whnfimp}{\imp^{\scriptscriptstyle{\Whnf}}}
\newcommand{\enfcompimp}{\imp^{\scriptscriptstyle{\Lambda}}}
\newcommand{\enfvalimp}{\imp^{\scriptscriptstyle{\Enf}}}
\newcommand{\whnfcompimp}{\imp^{\scriptscriptstyle{\Lambda}}}
\newcommand{\whnfvalimp}{\imp^{\scriptscriptstyle{\Whnf}}}


\newcommand{\ctximp}{\imp}
\newcommand{\ctxvalimp}{\valimp}

\newcommand{\approxsem}[2]{\sem{#1}_{#2}}
\newcommand{\howeimpcomp}{\models^{\mathsf{c}}}
\newcommand{\howeimpval}{\models^{\mathsf{v}}}
\newcommand{\fun}[2]{\bblambda#1.#2}
\newcommand{\alert}[1]{\textbf{#1}}

\newcommand{\varlambda}{\lambda}
\newcommand{\cpobot}{0}
\newcommand{\evalto}{\Downarrow}
\newcommand{\relonevalues}[1]{\relone_{#1}}
\newcommand{\reloneterms}[1]{\reltwo_{#1}}
\newcommand{\rec}[2]{\recType{#1}{#2}}
\newcommand{\lsimilarity}{\preceq}
\newcommand{\lsimilarityvalues}{\lsimilarity^{\values}}
\newcommand{\lsimilarityterms}{\lsimilarity^{\Lambda}}
\newcommand{\relimp}{\vdash}

\newcommand{\basisone}{\envone}
\newcommand{\basistwo}{\envtwo}
\newcommand{\substthree}{\vartheta}
\newcommand{\substfour}{\varsigma}
\newcommand{\applysubst}[2]{#1[#2]}
\newcommand{\reloneenv}[1]{\mathcal{Q}_{#1}}
%\newcommand{\defiff}{{\mathrel{\ensurestackMath{\stackon[1pt]{\iff}{\scriptstyle\triangle}}}}}
\newcommand{\defiff}{\iff^{def}}
%%%% OPERATIONAL SEMANTICS
\newcommand{\constone}{\omega}
\newcommand{\convergeconst}[1]{\downarrow_{#1}}
\newcommand{\smallstepeff}[1]{\overset{#1}{\longrightarrow}}
\newcommand{\smallstep}{\longrightarrow}
\newcommand{\multistep}{\Downarrow}


%%%% LANGUAGE
\newcommand{\Language}{\Lambda}
\newcommand{\lambdap}{\Lambda_{\probb}}
\newcommand{\lambdacont}{\Lambda_{\probb}^{c}}

%%% MONADS
\newcommand{\return}{\mathsf{return}}

%%% SEMANTICS %%%
\newcommand{\semn}[2]{\sem{#1}^{(#2)}}
\newcommand{\ocppo}{\ensuremath{\omega\text{-}\mathbf{cppo}}}

%%% Context equivalence:
\newcommand{\contset}{\mathfrak{C}}
\newcommand{\contfun}{\mathfrak{C}}
\newcommand{\ctxone}{\contfun}
\newcommand{\contexts}[1]{\contset_{#1}}
\newcommand{\hole}{[\cdot]}
\newcommand{\holefill}[1]{[#1]}

%% Measure theory
\newcommand{\borels}[1]{\text{Borel}(#1)}

%% Environments

\newenvironment{varitemize}
{
	\begin{list}{\longv{\labelitemi}\shortv{\labelitemi}}
		{\setlength{\itemsep}{0pt}
			\setlength{\topsep}{0pt}
			\setlength{\parsep}{0pt}
			\setlength{\partopsep}{0pt}
			\setlength{\leftmargin}{15pt}
			\setlength{\rightmargin}{0pt}
			\setlength{\itemindent}{0pt}
			\setlength{\labelsep}{5pt}
			\setlength{\labelwidth}{10pt}
	}}
	{
	\end{list} 
}

\newcounter{numberone}

\newenvironment{varenumerate}
{
	\begin{list}{\arabic{numberone}.}
		{
			\usecounter{numberone}
			\setlength{\itemsep}{0pt}
			\setlength{\topsep}{0pt}
			\setlength{\parsep}{0pt}
			\setlength{\partopsep}{0pt}
			\setlength{\leftmargin}{15pt}
			\setlength{\rightmargin}{0pt}
			\setlength{\itemindent}{0pt}
			\setlength{\labelsep}{5pt}
			\setlength{\labelwidth}{15pt}
	}}
	{
	\end{list} 
}

\newcommand{\kleisli}[1]{#1^{\dagger}}
\newcommand{\forward}[1]{#1_{\sharp}}
\newcommand{\converse}[1]{#1^-}
\newcommand{\unit}{\eta}
\newcommand{\relatortwo}{\Theta}

\newcommand{\statet}{\mathit{state}}
\newcommand{\event}{\mathit{event}}
\newcommand{\logic}{\mathit{logic}}
\newcommand{\test}{\mathit{test}}
\newcommand{\ctxeq}{\equiv^{\mathit{ctx}}}

